Measuring contact angle and meniscus shape with a reflected laser beam

Side-view imaging of the contact angle between an extended planar solid surface and a liquid is problematic. Even when aligning the view perfectly parallel to the contact line, focusing one point of the contact line is not possible. We describe a new measurement technique for determining contact angles with the reflection of a widened laser sheet on a moving contact line. We verified this new technique measuring the contact angle on a cylinder, rotating partially immersed in a liquid. A laser sheet is inclined under an angle $\varphi$ to the unperturbed liquid surface and is reflected off the meniscus. Collected on a screen, the reflection image contains information to determine the contact angle. When dividing the laser sheet into an array of laser rays by placing a mesh into the beam path, the shape of the meniscus can be reconstructed from the reflection image. We verified the method by measuring the receding contact angle versus speed for aqueous cetyltrimethyl ammonium bromide solutions on a smooth hydrophobized as well as on a rough polystyrene surface.

==> 2_Reflection_-_alt.tex <==
\section{Reflection of a laser beam on a meniscus}
\label{section_Measuring_contact_angle}
In a setup similar to the one used by Fell et al. \citep[][]{Fell2011, Fell2011_2}, a cylinder rotated in a liquid and caused a deformation of the liquid surface. With this setup they could determine the velocity dependent contact angle with side view imaging. We used a laser sheet to illuminate a line across the contact line and analyzed the reflection of this laser sheet. The reflections, collected on a screen, displayed a characteristic shape, from which the contact angle and the shape of the meniscus could be calculated.
%-------------------------------------------------------------------------------------------------------------------------


\subsection{Experimental setup}
\label{subsection_Experimental_setup}
\begin{figure}[t]
	\centering
	\includegraphics[width=8.5cm]{Bilder/Skizze_Aufbau}
	\caption[]{Schematic of the experimental setup. The cylinder was rotating in a bath filled with a liquid. A widened laser sheet with a wavelength of $\lambda = 635\,nm$ was inclined under an angle $\varphi$ to the liquid surface and was reflected on the cylinder (green dashed), the meniscus (red) and the unperturbed liquid surface (blue dotted). The reflection image was collected on a screen where the angle $\theta_{Refl}$ can be detected.}
	\label{Aufbau}
\end{figure}
\begin{figure}[t]
	\centering
	\includegraphics[width=5.5cm]{Bilder/Skizze_Aufbau_2}
	\caption[]{Schematic of the experimental setup. View from the side on the cylinder, rotating in the bath. The laser sheet is inclined under an angle $\varphi$ to the liquid surface.}
	\label{Aufbau}
\end{figure}\par
The setup was based on a bath, which was about $9\,cm$ in width, $15\,cm$ in depth, and $15\,cm$ in height, made out of polyvinyl chloride (PVC). In the bath, a horizontally oriented cylinder was rotating, driven by a motor with velocities ranging from $0.01\,cm/s$ up to $100\,cm/s$. The cylinder was made of stainless steel with a radius of $6\,cm$ and a length of $5\,cm$ (Fig. \ref{Aufbau}). Two different surfaces of the cylinder were used: the polished stainless steel surface and thin glass plates ($50\,mm \times 200\,mm \times 70\, \mu m$, kindly provided by Gerhard Menzel GmbH, 38116 Braunschweig, Germany) that were bent and glued on the cylinder. To hydrophobize the surfaces they were coated. The steel cylinder was coated with polystyrene. To do so, it rotated at a speed of $8\,cm/s$ in a $0.8\,wt\, \%$ solution of polystyrene ($M_w = 163\,kg/mol$) in tetrahydrofuran. Because of the evaporation of the solvent, a polystyrene film remained on the cylinder \citep[][]{Fell2011}. 
%The roughness for silanised glass was measured with an atomic force microscope (AFM) to be $\approx 1\, nm$ (RMS) on a surface of $25\mu m \times 25\mu m$\citep[][]{Fell2012}. 
To coat the glass plates with hexamethyldisilazane (HMDS), a solution of $2.5\,wt\, \%$ of hexamethyldisilazane ($M_w = 0.161\,kg/mol$) in toluene was used. When coating with hexamethyldisilazane the evaporation played no role, because it was bond chemically to the glass. The coatings were dried for 16 (polystyrene) and 3 hours (hexametyldisilazane) in the oven at $60\,^{\circ}C$, respectively, before being used for the wetting experiment. The roughnesses were measured with an atomic force microscope (AFM). For silanized glass the roughness was $\approx 1\, nm$ (RMS) on a surface of $25\mu m \times 25\mu m$. For PS on steel it was $167 \pm 38\,nm$ (RMS) on a surface of $50\mu m \times 50\mu m$ \citep[][]{Fell2012}.
%\begin{table}[h]
%\centering
%\begin{tabular}{l | l | l }
%	Surface & Coating & Roughness \\
%	\hline
%	Steel & PS & $167 \pm 38\,nm$ \\
%	Glass & HMDS & $1\,nm$ \\
%\end{tabular} 
%\caption[]{Listing of the used surfaces and the coatings with the specific roughnesses, measured with an atomic force microscope by Fell \citep[][]{Fell2012}.}
%\label{Tab_Surface}
%\end{table}
The bath was filled with a liquid, so that the cylinder was more than half immersed in it. The contact line between the cylinder and the liquid was illuminated by a laser (Lasiris SNF, Coherent, Santa Clara, CA 95006 USA) with a wavelength of $635\,nm$ and $10\,mW$ power. The laser beam was enlarged in one spatial direction by an optical lens generating a laser sheet with an opening angle of $\gamma = 10\,^{\circ}$ and a thickness of $d = 50 - 75\, \mu m$. The laser sheet was inclined under an angle $\varphi$ to the liquid surface where it hit the cylinder and the liquid surface. The laser sheet was oriented such that the central ray of the laser sheet and the normal to the laser sheet span a plane that was parallel to the x-z-plane (Fig. \ref{Aufbau}). To describe the reflection of the laser sheet, it is convenient to distinguish three different regions for the reflection (Fig. \ref{Reflektion_des_Lasers}): the cylinder surface (from A to B), the meniscus (B to C), and the plane liquid surface (C to D). The reflections hit a screen that was positioned behind the bath. The reflections were recorded with a camera (Olympus, i-Speed LT equipped with a SIGMA AF 50/2.8 DG Macro objective) with a maximum frame rate of $2000\, fps$.\par
%\begin{table}[h]
%\centering
%\begin{tabular}{l | l }
%	Parameter & Value \\
%	\hline
%	Bath width & $9\,cm$ \\
%	Bath hight & $15\,cm$ \\
%	Bath depth & $15\,cm$ \\
%	Cylinder radius & $6\,cm$ \\
%	Cylinder length & $5\,cm$ \\
%	Glass plate thickness & $70\, \mu m$ \\
%	Mesh: wire thickness & $63\, \mu m$ \\
%	Mesh: distance between the openings & $b=163\, \mu m$ \\
%	Distance between laser and mesh & $l_1=19.4\,cm$ \\
%	Distance between mesh and meniscus & $l_2=8.8\,cm$ \\
%	Laser wavelength & $635\,nm$ \\
%	Laser power & $10\,mW$ \\
%	Laser opening angle & $\gamma = 10\,^{\circ}$ \\
%	Laser thickness & $d = 50 - 75\, \mu m$ \\
%\end{tabular} 
%\caption[]{Listing of the geometrical parameters of the used setup.}
%\label{Tab_setup}
%\end{table}
Two liquids were used in the presented experiments: Milli-Q water and aqueous solutions of the cationic surfactant CTAB (cetyltrimethylammonium bromide; $\ce{CH3(CH2)15N+(CH3)3BR-}$, critical micelle concentration (cmc) $= 1\,mmol/l$). All experiments were carried out in a water saturated atmosphere.
\begin{figure}[t]
	\centering
	\includegraphics[width=8.5cm]{Bilder/Reflektion_des_Lasers}
	\caption[]{Schematic side-view of the rotating cylinder and the meniscus. The locations where the widened laser sheet is reflected are colored in green dashed (cylinder), red (meniscus) and blue dotted (unperturbed liquid surface).}
	\label{Reflektion_des_Lasers}
\end{figure}
For verification, contact angles were recorded with the side view method described by Fell et al. \citep[][]{Fell2011}.\par
To reconstruct the meniscus profile, the laser sheet was split up in single laser beams by placing a steal mesh (Haver \& Boecker, 59302 Oelde, Germany) in the laser sheet. The mesh consisted of woven steel wires with a thickness of $63\, \mu m$ and an opening of $100\, \mu m$, so that it had a distance between the openings of the mesh of $163\, \mu m$. This led to a group of individual rays being reflected from the meniscus.
%-------------------------------------------------------------------------------------------------------------------------


\subsection{Modeling with Geometrical Optics}
\label{subsection_theoretical}
We used geometrical optics to follow the beam path of the individual rays of the laser sheet. Deduced formulas relate the shape of the reflection to the contact angle and the shape of the meniscus. The used coordinate system is given in Fig. \ref{Aufbau}. Additional parameters are: the position of the laser $\vec{p} = \left( p_1, p_2, p_3 \right)$, the angle $\varphi$, under which the laser sheet is inclined to the liquid surface, the opening angle $\gamma$ of the laser sheet, the radius $r$ and the position of the cylinder, the reference point $\vec{q} = \left( q_1, q_2, q_3 \right)$ of the screen and its normal vector $\vec{n_S}$. Also the position of the unperturbed liquid surface must be known. When knowing these parameters, the laser sheet is represented by an array of rays (straight lines)
\begin{equation}
g_i: \vec{x} = \vec{p} + \lambda \vec{a_i}
\label{Gleichung_1}
\end{equation}
with the scaling parameter $\lambda$ and the direction vector
\begin{align}
\vec{a_i} = \left(\begin{array}{c} a_{i1} \\ a_{i2} \\ a_{i3} \end{array}\right)
 &= \left(\begin{array}{c} -\cos( \varphi ) \cdot \cos( \epsilon_i ) \\ \sin( \epsilon_i ) \\ -\sin( \varphi ) \cdot \cos( \epsilon_i ) \end{array}\right) \notag \\ &\approx \left(\begin{array}{c} -\cos( \varphi ) \\ \epsilon_i \\ -\sin( \varphi ) \end{array}\right)
\label{Gleichung_13}
\end{align}
that depends on the array index $i$. Here the last approximation is only valid for small opening angles of the laser sheet. In further calculations we focus on one ray and omit the index $i$ for clarity. Details of the calculation can be found in the Appendix \ref{section_Calculation2}.
%-------------------------------------------------------------------------------------------------------------------------


\subsection{Calculation of the contact angle}
\label{subsection_calculation}
\begin{figure}[t]
  \centering
  \subfigure[]{
    \label{Beispiel_1_1}
    \includegraphics[width=4cm]{Bilder/Beispiel_Profil}
  }
  \subfigure[]{
    \label{Beispiel_1_2}
    \includegraphics[width=4cm]{Bilder/Beispiel_Reflexion_Winkel}
  }
  \caption[]{(a) Side-view on the cylinder and the meniscus. With the reflection method the inclination angle $\alpha$ of the meniscus is calculated. Subtracting the inclination angle $\beta$ of the surface at the contact line, one receive the contact angle $\theta$. (b) From the reflection image the angle $\theta_{Refl}$ was determined for calculating the contact angle $\theta$.}
  \label{Beispiel_1}
\end{figure}
As detailed in Appendix \ref{section_Calculation2}, the slope $m_{Refl}$ of the meniscus reflection is related to the slope of the meniscus $m$ at the reflection point by
\begin{equation}
m_{Refl} = \frac{2m}{1-m^2}
\label{Gleichung_8}
\end{equation}
At the end point of the reflection, e.g., at the three phase contact line, we can rewrite this relation with the identities $m=-\frac{1}{\tan (\alpha )}$ and $m_{Refl}=\tan (\theta_{Refl} )$ (Fig. \ref{Beispiel_1}): 
\begin{equation}
\alpha = \frac{1}{2} \theta_{Refl}.
\label{Gleichung_9}
\end{equation}
For getting the contact angle $\theta$, the angle $\beta$ between the vertical line and the cylinder surface at the contact line must be taken into account
\begin{equation}
\theta = \alpha - \beta = \frac{1}{2} \theta_{Refl} - \beta.
\label{Gleichung_10}
\end{equation}
We analyzed the reflection images with a self written program in MATLAB. For an accurate positioning of the reflection, the position of all bright pixels belonging to the reflection were averaged horizontally. The resulting average shape of the reflection was fitted with a smooth function. At the end point of the reflection, the angle between the tangential and the horizontal line defines the angle $\theta_{Refl}$. Using Eq. (\ref{Gleichung_10}), we deduced the contact angle $\theta$ (Fig. \ref{Beispiel_1}). $\beta$ was easily measured directly from a side-view image of the cylinder or calculated from the filling height. For automatical analysis, a video with around $100$ frames was taken and the contact angles were calculated for every image. In the experimental part below, the contact angles for one video are averaged. The error represents the standard deviation.
%-------------------------------------------------------------------------------------------------------------------------


\subsection{Reconstruction of the meniscus profile}
\label{subsection_reconstruction}
For reconstructing the meniscus shape from the reflection, the laser sheet was split into single rays. They were reflected and generated a dotted reflection image. Every dot originated from the ray from one opening in the mesh (Fig. \ref{Meniscus_reconstruction_2}). The theoretical analysis did not change in this case. The angular distance between the rays was given by the distance between the openings in the mesh and the position of the mesh in the setup.
\begin{figure}[t]
  \centering
  \subfigure[]{
    \label{Meniscus_reconstruction_2}
    \includegraphics[width=4cm]{Bilder/Meniscus_Reconstruction}
  }
  \subfigure[]{
    \label{Meniscus_reconstruction_1}
    \includegraphics[width=4cm]{Bilder/Meniscus_Reconstruction_Reflection}
  }
  \caption[]{(a) Dotted reflection image with every dot belonging to a ray originating from one opening in the mesh. Two neighboring rays have an angular distance of $e \approx \arctan \left(\frac{b}{l_1} \right) \approx 0.0048\,^{\circ}$, with the distance between the openings of the mesh $b$ and the distance $l_1$ between laser and mesh. The rays reflected in the vicinity of the contact line were easily identifiable. Far away from the contact line the dots could not be separated and were not included in the reconstruction of the meniscus shape. (b) Side-view image superimposed with the reconstructed shape of the meniscus (black dots with white surrounding).}
  \label{Meniscus_reconstruction}
\end{figure}\par 
For calculating the contact angles, the reflections of the single rays on the screen must be located. This was done with the particle tracking-algorithm by Crocker, Grier, and Weeks \citep[][]{Crocker1996}, transferred to MATLAB by D. Blair and E. Dufresne \citep[][]{MATLAB2012}. The dots reflected close to the point C (and further away from the contact line) could not be separated in the image analysis and were not included in the reconstruction of the meniscus shape. The slope between two dots in the reflection image was determined to $m_{Refl}=\frac{\Delta z}{\Delta y}$. Eq. (\ref{Gleichung_8}) yields to the slope $m$ of the meniscus segment between the reflection points of these two rays. The distance on the meniscus between the central and another ray was calculated from the distance between laser and mesh $l_1$, between mesh and meniscus $l_2$ and the distance between the openings of the mesh $b$ to
\begin{equation}
c= \tan \left( \arctan \left( \frac{b \cdot (j-0.5}{l_1} \right) \right) \cdot \left( l_1 + l_2 \right).
%c=\tan \left( \sin \left( \frac{b(j-0.5)}{l_1+l_2} \right) \right),
\label{Gleichung_14}
\end{equation}
Here, $j$ describes the number of rays away from the central ray. To reconstruct the meniscus shape, we first determined the slope of all its segments. The shape of the meniscus was calculated as the piecewise linear function of these segments. Starting from the known y- and z-coordinates of the contact line, the shape was composed by calculating the length and the slope of each segment. The length of the first segment was chosen to be half of the following segments. For the latter ones the length of the segments is given by Eq. (\ref{Gleichung_14}). The end points of the segments are compared to the meniscus shape in Fig. \ref{Meniscus_reconstruction_1}.










